Lifts, transfers, and degrees of univariate maps

One can compute the local $\mathbb{A}^1$-degree at points with separable residue field by base changing, working rationally, and post-composing with the field trace. We show that for endomorphisms of the affine line, one can compute the local $\mathbb{A}^1$-degree at points with inseparable residue field by taking a suitable lift of the polynomial and transferring its local degree. We also discuss the general set-up and strategy in terms of the six functor formalism. As an application, we show that trace forms of number fields are local $\mathbb{A}^1$-degrees.

==> commands.tex <==
% Packages
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{amsfonts}
%\RequirePackage{geometry}
\RequirePackage{color}
\RequirePackage{mathtools}
\RequirePackage{bbm}
\RequirePackage{amsfonts}
\RequirePackage{mathrsfs}
\RequirePackage{tikz}
\usepackage[shortlabels]{enumitem}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{cd}
\tikzstyle{arrow} = [thick,->,>=stealth]

% Arrows
\providecommand{\po}{\arrow[ul,phantom,"\ulcorner" very near start]}
\providecommand{\pb}{\arrow[dr,phantom,"\lrcorner" very near start]}
\providecommand{\xto}[1]{\xrightarrow{#1}}
\providecommand{\from}{\leftarrow}
\providecommand{\xfrom}[1]{\overset{#1}{\leftarrow}}

\providecommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\providecommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}

\providecommand{\hookto}{\xhookrightarrow{}}
\providecommand{\xhookto}[1]{\overset{#1}{\hookrightarrow}}

\providecommand{\hookfrom}{\xhookleftarrow{}}
\providecommand{\xhookfrom}[1]{\xhookleftarrow{#1}}

\providecommand{\tto}{\twoheadrightarrow}
\providecommand{\xtto}[1]{\overset{#1}{\twoheadrightarrow}}
\providecommand{\ffrom}{\twoheadleftarrow}
\providecommand{\xffrom}[1]{\overset{#1}{\ffrom}}

\providecommand{\ladjoint}[2]{ #1\rightleftarrows #2 }
\makeatletter
\providecommand{\superimpose}[2]{%
  {\ooalign{$#1\@firstoftwo#2$\cr\hfil$#1\@secondoftwo#2$\hfil\cr}}}
\makeatother
\providecommand{\smallslash}{\mbox{\tiny/}}

\providecommand{\clhookto}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookrightarrow}}}$}}}
\providecommand{\xclhook}[1]{\overset{#1}{\clhook}}

\providecommand{\clhookfrom}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookleftarrow}}}$}}}

\providecommand{\ohookto}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookrightarrow}}}$}}}

\providecommand{\ohookfrom}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookleftarrow}}}$}}}

\providecommand{\cofto}{\rightarrowtail}
\providecommand{\coffrom}{\leftarrowtail}
\providecommand{\xcofto}[1]{\overset{#1}{\cofto}}
\providecommand{\xcoffrom}[1]{\overset{#1}{\coffrom}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

% Common Text Commands
\providecommand{\ab}{\text{ab}}
\providecommand{\ann}{\text{ann}}
\providecommand{\Aut}{\text{Aut}}
\providecommand{\char}{\text{char}}
\providecommand{\cl}{\text{cl}}
\providecommand{\codim}{\text{codim}}
\providecommand{\colim}{\text{colim}}
\providecommand{\conj}{\text{conj}}
\providecommand{\const}{\text{const}}
\providecommand{\Disc}{\text{Disc}}
\providecommand{\End}{\text{End}}
\providecommand{\EKL}{\text{EKL}}
\providecommand{\ev}{\text{ev}}
\providecommand{\Fix}{\text{Fix}}
\providecommand{\Frac}{\text{Frac}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Fun}{\text{Fun}}
\providecommand{\Gal}{\text{Gal}}
\providecommand{\GL}{\text{GL}}
\providecommand{\gr}{\text{gr}}
\newcommand{\GW}{\text{GW}}
\providecommand{\Hom}{\text{Hom}}
\providecommand{\id}{\text{id}}
\providecommand{\im}{\text{im}}
\renewcommand{\Im}{\text{Im}}
\providecommand{\incl}{\text{incl}}
\providecommand{\Ind}{\text{Ind}}
\providecommand{\Inn}{\text{Inn}}
\providecommand{\Jac}{\text{Jac}}
\providecommand{\Map}{\text{Map}}
\providecommand{\mult}{\text{mult}}
\providecommand{\op}{\text{op}}
\providecommand{\Orb}{\text{Orb}}
\providecommand{\ord}{\text{ord}}
\providecommand{\Out}{\text{Out}}
\providecommand{\Perm}{\text{Perm}}
\providecommand{\pr}{\text{pr}}
\providecommand{\pre}{\text{pre}}
\providecommand{\PSL}{\text{PSL}}
\providecommand{\quot}{\text{quot}}
\providecommand{\rank}{\text{rank}}
\renewcommand{\Re}{\text{Re}}
\providecommand{\Res}{\text{Res}}
\providecommand{\sgn}{\text{sgn}}
\providecommand{\sig}{\text{sig}}
\providecommand{\SL}{\text{SL}}
\providecommand{\soc}{\text{soc}}
\providecommand{\spn}{\text{span}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\Stab}{\text{Stab}}
\providecommand{\supp}{\text{supp}}
\providecommand{\Syl}{\text{Syl}}
\providecommand{\syl}{\text{syl}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\Tor}{\text{Tor}}
\providecommand{\Tr}{\text{Tr}}

% BB Sets
\providecommand{\A}{\mathbb{A}}
\providecommand{\C}{\mathbb{C}}
\providecommand{\F}{\mathbb{F}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\P}{\mathbb{P}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\Z}{\mathbb{Z}}

% Commands
\providecommand{\lrangle}[1]{\left\langle #1 \right\rangle}
\providecommand{\nsubgp}{\trianglelefteq}
\providecommand{\p}{\mathfrak{p}}
\renewcommand{\H}{\textbf{H}}
\newcommand{\gw}[1]{\left\langle #1 \right\rangle}
\newcommand{\ovl}[1]{\overline{#1}}

\let\minus\smallsetminus
\let\bar\overline
\let\smsh\wedge

\providecommand{\SH}{\mathcal{SH}}


% Colors
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\red}[1]{\textcolor{red}{#1}}
\providecommand{\orange}[1]{\textcolor{orange}{#1}}
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\blue}[1]{\textcolor{blue}{#1}}
\providecommand{\purple}[1]{\textcolor{purple}{#1}}

